Smoothed Separable Nonnegative Matrix Factorization

Given a set of data points belonging to the convex hull of a set of vertices, a key problem in linear algebra, signal processing, data analysis and machine learning is to estimate these vertices in the presence of noise. Many algorithms have been developed under the assumption that there is at least one nearby data point to each vertex; two of the most widely used ones are vertex component analysis (VCA) and the successive projection algorithm (SPA). This assumption is known as the pure-pixel assumption in blind hyperspectral unmixing, and as the separability assumption in nonnegative matrix factorization. More recently, Bhattacharyya and Kannan (ACM-SIAM Symposium on Discrete Algorithms, 2020) proposed an algorithm for learning a latent simplex (ALLS) that relies on the assumption that there is more than one nearby data point to each vertex. In that scenario, ALLS is probalistically more robust to noise than algorithms based on the separability assumption. In this paper, inspired by ALLS, we propose smoothed VCA (SVCA) and smoothed SPA (SSPA) that generalize VCA and SPA by assuming the presence of several nearby data points to each vertex. We illustrate the effectiveness of SVCA and SSPA over VCA, SPA and ALLS on synthetic data sets, on the unmixing of hyperspectral images, and on feature extraction on facial images data sets. In addition, our study highlights new theoretical results for VCA.

==> xp/xpfaces.tex <==
\begin{table}[ht!]
\caption{Relative reconstruction errors ($\min_{H \geq 0} \| X - WH \|_F / \| X \|_F$) in percent resulting from the processing of facial image datasets with ALLS, SVCA, and SSPA, with different values of parameter $p$. SVCA(1) and SSPA(1) are equivalent to VCA and SPA. For non-deterministic algorithms ALLS and SVCA, we show the minimum, median, standard deviation, and maximum of the error over 30 trials.}
\centering
\begin{tabular}{ll|ccc|ccc}
     &    & \multicolumn{3}{c|}{CBCL}                & \multicolumn{3}{c}{Frey}                 \\
     & p  & Min     & Med $\pm$ std        & Max     & Min     & Med $\pm$ std        & Max     \\ \hline
ALLS & 1  & 19.36 & 20.08 $\pm$ 0.33 & 20.95 & 21.05 & 22.38 $\pm$ 0.58 & 23.83 \\
     & 5  & \textbf{18.53} & 19.60 $\pm$ 0.51 & 20.41 & \textbf{20.75} & \textbf{22.32} $\pm$ 0.73 & 23.96 \\
     & 10 & 18.67 & \textbf{19.44} $\pm$ 0.78 & 21.88 & 21.30 & 22.85 $\pm$ 0.85 & 24.57 \\
     & 20 & 19.34 & 20.28 $\pm$ 1.17 & 23.83 & 22.30 & 24.05 $\pm$ 1.10 & 27.42 \\ \hline
SVCA & 1  & 19.25 & 19.81 $\pm$ 0.31 & 20.48 & 20.99 & 22.18 $\pm$ 0.64 & 24.02 \\
     & 5  & 18.72 & 19.21 $\pm$ 0.34 & 20.14 & 20.69 & 21.57 $\pm$ 0.52 & 22.85 \\
     & 10 & 18.48 & \textbf{18.84} $\pm$ 0.35 & 19.76 & \textbf{20.68} & \textbf{21.29} $\pm$ 0.43 & 22.57 \\
     & 20 & \textbf{18.44} & 18.95 $\pm$ 0.25 & 19.55 & 20.79 & 21.70 $\pm$ 0.45 & 22.71 \\ \hline
SSPA & 1  & \multicolumn{3}{c|}{20.76}             & \multicolumn{3}{c}{22.57}              \\
     & 5  & \multicolumn{3}{c|}{20.05}             & \multicolumn{3}{c}{21.65}              \\
     & 10 & \multicolumn{3}{c|}{\textbf{19.63}}             & \multicolumn{3}{c}{\textbf{21.32}}              \\
     & 20 & \multicolumn{3}{c|}{20.83}             & \multicolumn{3}{c}{21.58}             \\
     & & & & & & & \\ \hline
          &     & \multicolumn{3}{c|}{ORL}         & \multicolumn{3}{c}{Umist}        \\
     & p   & Min   & Med $\pm$ std    & Max   & Min   & Med $\pm$ std    & Max   \\ \hline
ALLS & 1   & 23.64 & 24.08 $\pm$ 0.18 & 24.35 & 15.38 & 16.00 $\pm$ 0.25 & 16.46 \\
     & 50  & \textbf{22.87} & \textbf{23.62} $\pm$ 0.42 & 24.92 & \textbf{15.34} & \textbf{15.91} $\pm$ 0.32 & 16.48 \\
     & 200 & 23.34 & 24.33 $\pm$ 0.60 & 25.93 & 16.27 & 16.96 $\pm$ 0.54 & 18.87 \\
     & 400 & 24.50 & 25.31 $\pm$ 0.45 & 26.56 & 17.28 & 18.21 $\pm$ 0.49 & 19.07 \\ \hline
SVCA & 1   & 23.34 & 24.04 $\pm$ 0.32 & 24.70 & 15.40 & 15.95 $\pm$ 0.24 & 16.28 \\
     & 50  & 22.31 & 22.89 $\pm$ 0.32 & 23.63 & 14.95 & \textbf{15.37} $\pm$ 0.28 & 16.08 \\
     & 200 & \textbf{22.22} & \textbf{22.70} $\pm$ 0.29 & 23.53 & \textbf{14.90} & \textbf{15.37} $\pm$ 0.25 & 15.91 \\
     & 400 & 22.42 & 23.00 $\pm$ 0.34 & 23.86 & 15.29 & 15.85 $\pm$ 0.30 & 16.46 \\ \hline
SSPA & 1   & \multicolumn{3}{c|}{25.76}     & \multicolumn{3}{c}{16.56}      \\
     & 50  & \multicolumn{3}{c|}{24.14}     & \multicolumn{3}{c}{15.72}      \\
     & 200 & \multicolumn{3}{c|}{\textbf{23.50}}     & \multicolumn{3}{c}{\textbf{14.98}}      \\
     & 400 & \multicolumn{3}{c|}{24.50}     & \multicolumn{3}{c}{15.40} 
\end{tabular}%
\label{tab:xpfaces1}
\end{table}

==> xp/xphsu.tex <==
\begin{table*}[ht]
\caption{Relative reconstruction errors ($\min_{H \geq 0} \| X - WH \|_F / \| X \|_F$) resulting from the unmixing of hyperspectral images with ALLS, SVCA, and SSPA, with different values of parameter $p$. SVCA(1) and SSPA(1) are equivalent to VCA and SPA. For non-deterministic algorithms ALLS and SVCA, we show the minimum, median, standard deviation, and maximum of the error over 30 trials.}
\label{tab:xphsu}
\resizebox{\textwidth}{!}{%
\centering
\begin{tabular}{ll|ccc|ccc|ccc}
     &      & \multicolumn{3}{c|}{SanDiego}  & \multicolumn{3}{c|}{Urban}      & \multicolumn{3}{c}{Terrain}  \\
     & p    & Min  & Med $\pm$ std   & Max   & Min  & Med $\pm$ std    & Max   & Min  & Med $\pm$ std   & Max  \\ \hline
ALLS & 1    & 4.72 & 5.60 $\pm$ 0.67 & 8.25  & 5.39 & 9.14 $\pm$ 1.93  & 12.26 & 3.94 & 4.88 $\pm$ 0.73 & 7.08 \\
     & 100  & \textbf{4.27} & \textbf{5.35} $\pm$ 1.72 & 10.91 & \textbf{6.37} & \textbf{9.28} $\pm$ 3.18  & 19.40 & \textbf{3.84} & 4.87 $\pm$ 0.87 & 6.85 \\
     & 1000 & 4.64 & 6.14 $\pm$ 1.12 & 8.68  & 6.78 & 9.71 $\pm$ 2.16  & 14.20 & \textbf{3.84} & \textbf{4.71} $\pm$ 1.19 & 8.81 \\
     & 2000 & 4.87 & 5.91 $\pm$ 1.62 & 11.79 & 6.96 & 9.93 $\pm$ 1.60  & 12.85 & 3.96 & 4.89 $\pm$ 0.88 & 7.63 \\
     & 5000 & 5.51 & 7.42 $\pm$ 2.64 & 13.88 & 7.68 & 10.37 $\pm$ 1.89 & 14.98 & 4.28 & 5.26 $\pm$ 0.80 & 6.88 \\ \hline
SVCA & 1    & 3.95 & 5.42 $\pm$ 0.61 & 6.90  & 6.25 & 9.13 $\pm$ 1.78  & 12.23 & 4.03 & 5.11 $\pm$ 1.25 & 8.70 \\
     & 100  & \textbf{3.44} & 4.92 $\pm$ 0.77 & 6.96  & \textbf{5.08} & \textbf{6.10} $\pm$ 1.27  & 10.13 & 3.52 & 4.04 $\pm$ 0.67 & 6.52 \\
     & 1000 & 3.82 & 4.95 $\pm$ 0.59 & 6.82  & 5.82 & 6.77 $\pm$ 1.23  & 10.84 & \textbf{3.18} & \textbf{3.92} $\pm$ 0.38 & 4.70 \\
     & 2000 & 3.73 & \textbf{4.40} $\pm$ 0.51 & 5.81  & 5.66 & 6.36 $\pm$ 0.67  & 7.83  & 3.38 & 4.12 $\pm$ 0.45 & 4.95 \\
     & 5000 & 4.01 & 4.66 $\pm$ 0.73 & 7.01  & 5.69 & 6.94 $\pm$ 1.21  & 11.74 & 3.70 & 4.19 $\pm$ 0.30 & 4.82 \\ \hline
SSPA & 1    & \multicolumn{3}{c|}{5.90}      & \multicolumn{3}{c|}{9.46}       & \multicolumn{3}{c}{5.01}     \\
     & 100  & \multicolumn{3}{c|}{9.29}      & \multicolumn{3}{c|}{6.65}       & \multicolumn{3}{c}{\textbf{4.03}}     \\
     & 1000 & \multicolumn{3}{c|}{5.82}      & \multicolumn{3}{c|}{6.22}       & \multicolumn{3}{c}{8.05}     \\
     & 2000 & \multicolumn{3}{c|}{\textbf{4.32}}      & \multicolumn{3}{c|}{6.11}       & \multicolumn{3}{c}{7.86}     \\
     & 5000 & \multicolumn{3}{c|}{4.65}      & \multicolumn{3}{c|}{\textbf{5.91}}       & \multicolumn{3}{c}{5.38}   
\end{tabular}%
}
\end{table*}



%%%% Old table with preprocess and Cuprite
% \begin{tabular}{ll|ccc|ccc|ccc|ccc|}
%      &      & \multicolumn{3}{c|}{Cuprite}  & \multicolumn{3}{c|}{SanDiego}  & \multicolumn{3}{c|}{Urban}      & \multicolumn{3}{c|}{Terrain}  \\
%      & p    & Min  & Med $\pm$ std   & Max  & Min  & Med $\pm$ std   & Max   & Min  & Med $\pm$ std    & Max   & Min  & Med $\pm$ std   & Max  \\ \hline
% ALLS & 1    & 1.49 & 1.90 $\pm$ 0.72 & 4.70 & 4.72 & 5.60 $\pm$ 0.67 & 8.25  & 5.39 & 9.14 $\pm$ 1.93  & 12.26 & 3.94 & 4.88 $\pm$ 0.73 & 7.08 \\
%      & 100  & 1.73 & 2.40 $\pm$ 0.79 & 5.24 & 4.27 & 5.35 $\pm$ 1.72 & 10.91 & 6.37 & 9.28 $\pm$ 3.18  & 19.40 & 3.84 & 4.87 $\pm$ 0.87 & 6.85 \\
%      & 1000 & 2.21 & 2.56 $\pm$ 0.75 & 5.39 & 4.64 & 6.14 $\pm$ 1.12 & 8.68  & 6.78 & 9.71 $\pm$ 2.16  & 14.20 & 3.84 & 4.71 $\pm$ 1.19 & 8.81 \\
%      & 2000 & 2.64 & 3.40 $\pm$ 0.72 & 5.83 & 4.87 & 5.91 $\pm$ 1.62 & 11.79 & 6.96 & 9.93 $\pm$ 1.60  & 12.85 & 3.96 & 4.89 $\pm$ 0.88 & 7.63 \\
%      & 5000 &      &                 &      & 5.51 & 7.42 $\pm$ 2.64 & 13.88 & 7.68 & 10.37 $\pm$ 1.89 & 14.98 & 4.28 & 5.26 $\pm$ 0.80 & 6.88 \\ \hline
% SVCA & 1    & 1.60 & 1.89 $\pm$ 1.15 & 5.57 & 3.95 & 5.42 $\pm$ 0.61 & 6.90  & 6.25 & 9.13 $\pm$ 1.78  & 12.23 & 4.03 & 5.11 $\pm$ 1.25 & 8.70 \\
%      & 100  & 1.57 & 1.81 $\pm$ 0.37 & 3.41 & 3.44 & 4.92 $\pm$ 0.77 & 6.96  & 5.08 & 6.10 $\pm$ 1.27  & 10.13 & 3.52 & 4.04 $\pm$ 0.67 & 6.52 \\
%      & 1000 & 1.82 & 2.03 $\pm$ 0.17 & 2.49 & 3.82 & 4.95 $\pm$ 0.59 & 6.82  & 5.82 & 6.77 $\pm$ 1.23  & 10.84 & 3.18 & 3.92 $\pm$ 0.38 & 4.70 \\
%      & 2000 & 2.12 & 2.47 $\pm$ 0.20 & 3.10 & 3.73 & 4.40 $\pm$ 0.51 & 5.81  & 5.66 & 6.36 $\pm$ 0.67  & 7.83  & 3.38 & 4.12 $\pm$ 0.45 & 4.95 \\
%      & 5000 &      &                 &      & 4.01 & 4.66 $\pm$ 0.73 & 7.01  & 5.69 & 6.94 $\pm$ 1.21  & 11.74 & 3.70 & 4.19 $\pm$ 0.30 & 4.82 \\ \hline
% SSPA & 1    & \multicolumn{3}{c|}{1.84}     & \multicolumn{3}{c|}{5.90}      & \multicolumn{3}{c|}{9.46}       & \multicolumn{3}{c|}{5.01}     \\
%      & 100  & \multicolumn{3}{c|}{3.98}     & \multicolumn{3}{c|}{9.29}      & \multicolumn{3}{c|}{6.65}       & \multicolumn{3}{c|}{4.03}     \\
%      & 1000 & \multicolumn{3}{c|}{1.92}     & \multicolumn{3}{c|}{5.82}      & \multicolumn{3}{c|}{6.22}       & \multicolumn{3}{c|}{8.05}     \\
%      & 2000 & \multicolumn{3}{c|}{2.22}     & \multicolumn{3}{c|}{4.32}      & \multicolumn{3}{c|}{6.11}       & \multicolumn{3}{c|}{7.86}     \\
%      & 5000 & \multicolumn{3}{c|}{}         & \multicolumn{3}{c|}{4.65}      & \multicolumn{3}{c|}{5.91}       & \multicolumn{3}{c|}{5.38}    
% \end{tabular}



%%%% Below is old table with no preprocessing
% \begin{tabular}{ll|ccc|ccc|ccc|ccc}
%      &      & \multicolumn{3}{c|}{Cuprite} & \multicolumn{3}{c|}{SanDiego} & \multicolumn{3}{c|}{Urban}   & \multicolumn{3}{c}{Terrain} \\
%      & p    & Min   & Med $\pm$ std    & Max  & Min   & Med $\pm$ std    & Max   & Min  & Med $\pm$ std    & Max   & Min   & Med $\pm$ std   & Max  \\ \hline
% ALLS & 1    & 1.55  & 1.83 $\pm$ 1.16  & 5.38 & 7.93  & 10.25 $\pm$ 1.95 & 12.80 & 5.71 & 9.40 $\pm$ 1.21  & 9.85  & 4.13  & 5.24 $\pm$ 0.81 & 6.75 \\
%      & 100  & 1.78  & 2.63 $\pm$ 0.95  & 4.84 & 9.99  & 13.91 $\pm$ 1.44 & 15.77 & 5.71 & 10.10 $\pm$ 3.80 & 20.22 & 3.81  & 4.93 $\pm$ 1.04 & 6.96 \\
%      & 1000 & 2.21  & 3.15 $\pm$ 0.74  & 4.32 & 6.80  & 7.59 $\pm$ 0.94  & 9.92  & 7.18 & 9.54 $\pm$ 2.40  & 14.97 & 3.83  & 4.58 $\pm$ 1.12 & 8.62 \\
%      & 2000 & 2.66  & 3.64 $\pm$ 0.70  & 5.01 & 6.32  & 8.21 $\pm$ 1.27  & 11.22 & 7.16 & 9.44 $\pm$ 1.54  & 13.03 & 3.96  & 4.95 $\pm$ 0.96 & 7.52 \\
%      & 5000 &       &                  &      & 6.75  & 8.90 $\pm$ 1.88  & 13.93 & 7.88 & 9.82 $\pm$ 1.80  & 14.52 & 4.29  & 5.23 $\pm$ 0.76 & 6.81 \\ \hline
% SVCA & 1    & 1.52  & 1.76 $\pm$ 1.18  & 5.06 & 7.29  & 9.46 $\pm$ 2.23  & 16.25 & 5.79 & 9.58 $\pm$ 1.70  & 11.53 & 4.17  & 5.03 $\pm$ 0.69 & 6.32 \\
%      & 100  & 1.45  & 1.76 $\pm$ 0.29  & 2.58 & 5.98  & 6.64 $\pm$ 1.52  & 13.16 & 5.67 & 6.30 $\pm$ 1.50  & 10.27 & 3.56  & 4.27 $\pm$ 0.69 & 6.53 \\
%      & 1000 & 1.74  & 1.99 $\pm$ 0.15  & 2.27 & 5.66  & 6.13 $\pm$ 0.41  & 7.25  & 5.63 & 6.60 $\pm$ 0.73  & 8.22  & 3.50  & 4.02 $\pm$ 0.34 & 4.59 \\
%      & 2000 & 2.10  & 2.30 $\pm$ 0.12  & 2.52 & 5.88  & 6.23 $\pm$ 0.35  & 6.99  & 5.76 & 6.27 $\pm$ 0.63  & 7.74  & 3.68  & 4.14 $\pm$ 0.37 & 4.96 \\
%      & 5000 &       &                  &      & 6.05  & 6.28 $\pm$ 0.68  & 9.05  & 6.15 & 6.81 $\pm$ 0.75  & 9.08  & 3.71  & 4.23 $\pm$ 0.31 & 4.82 \\ \hline
% SSPA & 1    & \multicolumn{3}{c|}{1.74}    & \multicolumn{3}{c|}{12.68}    & \multicolumn{3}{c|}{9.58}    & \multicolumn{3}{c}{4.81}    \\
%      & 100  & \multicolumn{3}{c|}{1.47}    & \multicolumn{3}{c|}{15.83}    & \multicolumn{3}{c|}{7.59}    & \multicolumn{3}{c}{4.30}    \\
%      & 1000 & \multicolumn{3}{c|}{1.81}    & \multicolumn{3}{c|}{28.86}    & \multicolumn{3}{c|}{6.09}    & \multicolumn{3}{c}{6.96}    \\
%      & 2000 & \multicolumn{3}{c|}{2.19}    & \multicolumn{3}{c|}{28.58}    & \multicolumn{3}{c|}{5.86}    & \multicolumn{3}{c}{6.96}    \\
%      & 5000 & \multicolumn{3}{c|}{}        & \multicolumn{3}{c|}{26.15}    & \multicolumn{3}{c|}{6.11}    & \multicolumn{3}{c}{7.12}   
% \end{tabular}


%% Below is old table with sum-to-one constraint

% \begin{table}[ht]
% \caption{TODO caption}
% \label{tab:xphsu}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{ll|ccc|ccc|ccc|ccc}
%      &      & \multicolumn{3}{c|}{Cuprite} & \multicolumn{3}{c|}{SanDiego} & \multicolumn{3}{c|}{Urban} & \multicolumn{3}{c}{Terrain} \\
%      & p    & Min      & Med     & Max     & Min      & Med      & Max     & Min     & Med     & Max    & Min     & Med     & Max     \\ \hline
% ALLS & 1    & 1.57     & 1.84    & 5.39    & 7.93     & 10.25    & 12.80   & 5.72    & 9.40    & 9.85   & 4.13    & 5.28    & 6.77    \\
%      & 100  & 2.09     & 2.85    & 4.91    & 10.50    & 14.27    & 16.04   & 5.95    & 10.26   & 20.34  & 3.99    & 5.07    & 7.12    \\
%      & 1000 & 3.16     & 4.40    & 5.92    & 8.24     & 9.05     & 11.40   & 8.62    & 10.89   & 15.72  & 4.16    & 5.10    & 8.80    \\
%      & 2000 & 4.21     & 5.58    & 7.37    & 8.24     & 9.90     & 12.49   & 9.19    & 11.15   & 14.44  & 4.55    & 5.44    & 9.64    \\
%      & 5000 &          &         &         & 9.39     & 11.24    & 16.35   & 11.14   & 12.76   & 16.38  & 5.56    & 6.13    & 8.87    \\ \hline
% SVCA & 1    & 1.53     & 1.77    & 5.06    & 7.29     & 9.47     & 16.25   & 5.88    & 9.58    & 11.53  & 4.17    & 5.07    & 6.39    \\
%      & 100  & 1.65     & 1.99    & 2.75    & 6.90     & 7.74     & 13.53   & 5.98    & 6.71    & 10.41  & 3.69    & 4.32    & 6.57    \\
%      & 1000 & 2.84     & 3.00    & 3.93    & 7.77     & 8.17     & 8.88    & 7.51    & 8.46    & 10.66  & 3.88    & 4.34    & 4.89    \\
%      & 2000 & 4.08     & 4.82    & 5.71    & 8.20     & 8.48     & 9.38    & 8.30    & 8.72    & 14.22  & 4.18    & 4.74    & 6.05    \\
%      & 5000 &          &         &         & 9.13     & 9.61     & 11.69   & 10.39   & 11.09   & 13.18  & 4.71    & 5.25    & 6.95    \\ \hline
% SSPA & 1    & \multicolumn{3}{c|}{1.75}    & \multicolumn{3}{c|}{12.68}    & \multicolumn{3}{c|}{9.58}  & \multicolumn{3}{c}{4.81}    \\
%      & 100  & \multicolumn{3}{c|}{1.64}    & \multicolumn{3}{c|}{17.58}    & \multicolumn{3}{c|}{7.89}  & \multicolumn{3}{c}{4.36}    \\
%      & 1000 & \multicolumn{3}{c|}{2.85}    & \multicolumn{3}{c|}{29.13}    & \multicolumn{3}{c|}{7.86}  & \multicolumn{3}{c}{7.05}    \\
%      & 2000 & \multicolumn{3}{c|}{4.06}    & \multicolumn{3}{c|}{28.92}    & \multicolumn{3}{c|}{8.28}  & \multicolumn{3}{c}{7.12}    \\
%      & 5000 & \multicolumn{3}{c|}{}        & \multicolumn{3}{c|}{26.74}    & \multicolumn{3}{c|}{10.35} & \multicolumn{3}{c}{7.56}   
% \end{tabular}%
% }
% \end{table}
